Incentivizing Federated Learning

Federated Learning is an emerging distributed collaborative learning paradigm used by many of applications nowadays. The effectiveness of federated learning relies on clients' collective efforts and their willingness to contribute local data. However, due to privacy concerns and the costs of data collection and model training, clients may not always contribute all the data they possess, which would negatively affect the performance of the global model. This paper presents an incentive mechanism that encourages clients to contribute as much data as they can obtain. Unlike previous incentive mechanisms, our approach does not monetize data. Instead, we implicitly use model performance as a reward, i.e., significant contributors are paid off with better models. We theoretically prove that clients will use as much data as they can possibly possess to participate in federated learning under certain conditions with our incentive mechanism

==> src/old2_algorithm.tex <==
\section{Problem Formulation}

We first introduce some notations in traditional federated learning. Here, $C$ refers to the set of all the clients. $D^k$ denotes the local dataset of client $k\in C$ with $n_k$ samples. $\mathcal{D} = \bigcup_{k\in \mathcal{C}} \mathcal{D}^k$ represents the full training set. For an arbitrary set of clients $\mathcal{C}'$,

$\mathcal{L}(w, \mathcal{D}^k) = \frac{1}{n_k} \sum_{z\in \mathcal{D}^k} \mathcal{L}(w, z)$ denotes the empirical loss over a model $w$ and $D^k$. Then, the optimization problem of federated learning can be formulated as follow: 

\subsection{Traditional Federated Learning}
optimization problem:

\begin{equation}
    \min\limits_{w\in \R_p} \mathcal{L}(w, \mathcal{D}) = \sum\limits_{k\in \mathcal{C}_t} \frac{n_k}{N(\mathcal{C}_t)} 
    \mathcal{L}(w, \mathcal{D}^k)
\end{equation}
The global loss function

where the global loss function $\mathcal{L}(w, D)$ is the weighted average of the local functions $\mathcal{L}(w, \mathcal{D}^k)$ with the weight of each client proportioning to the size of its local dataset. In this work, we consider a standard algorithm, federated averaging (FedAvg), to solve the optimization problem.  FedAvg is the first and most widely used one. As a result, we see FedAvg as our basic block, which executes as follows In the initial stage, the server randomly initializes a global model $w_0$. Then, the training is orchestrated by repeating the following two steps for communication round $t$ from $1$ to $T$:

In federated learning, 

local training:
\begin{equation}
    w^k_{t,i}= w^k_{t,i-1} -  \eta \nabla \mathcal{L}(w^k_{t,i-1}, \mathcal{D}^k )
\end{equation}

Federated Averaging:
\begin{equation}
    w_t \leftarrow \sum\limits_{k\in \mathcal{C}_t} \frac{n_k}{N(\mathcal{C}_t)} w^k_{t,m}
\end{equation}

The idea of using client to model

Core idea: 
    1.better client model needs to aggregate together with other good client models, also needs them to be close in some metrics
    2. To further increase the discrepancy of the reward, allow better client models to aggregate with more other models.
    

\section{Main Approach}

Our main goal is to maximize the utility of every client. 

In traditional federated learning, there is an internal assumption that client's utility is only composed of the performance or performance improvement of the model they obtained from the centralized server.

However, we believe such assumption is not proper when moral hazard is considered. Specifically, every client could potentially contribute very little data or maybe use some fake data to train a local model to participate the federated learning, followed by a fine tuning over his own real data. In this way, the client could almost get all the benefits while contributing the least data or good model. If every client do that, the federation becomes meaningless since centralized server collects a bunch of garbage models. As a result, the federated learning becomes similar to individual machine learning. 

(if fake data, could that negatively affect the model performance? how should we model it in our framework.)

A incentive mechanism encourages clients to participate with as much data as possible. 



\begin{comment}
skeleton:
Motivation:
    Must incentivize, otherwise, will not come.
How to incentivize: 
    Goal: better clients would be rewarded with a better model.
    Side goal: ensure data segregation, better clients are willing to collaborate with other good clients.
    Core idea: 
    1.better client model needs to aggregate together with other good client models, also needs them to be close in some metrics
    2. To further increase the discrepancy of the reward, allow better client models to aggregate with more other model.
    
    Two important problems:
    1. How to decide good data/model contribution? what metrics to use for neighborhood selection.
    2. How to aggregate.
    
    two cases: 
    1. no validation dataset (graph, neighthood selection): hard to decide good or bad, can only do neighborhood through model similarity.
    2. has validation dataset. (ranking)
    can rank the model according to their performance on validation dataset. Better model will do a more smoother aggregate(smaller aggregation weight decay), worse model should do a more steep aggregation(mostly focus on itself), also, better model has larger aggregation range/spectrum.

Theory part:
     Use simplified model to show it.
    
    Utility function of the client: performance of the received model.(maybe a better one is increase of the performance, but hard to prove right now)
    
    Each client will try to maximize their utility, (try to maximize the performance of the received model)
    
    theorem: if they use all the data, their utility reaches maximum.
    
    Proof skeleton/idea: if they use more data, their model is better
    Then, after sent to server, during the aggregation, their model is supposed to aggregate with other better model in a more smoother way, thus their model is even better.
    
    same client:
    p1: local performance when use less data
    g1: global performance after aggregation when using less data.
    
    p2: same local performance when use more data
    g2: same global performance after aggregation when using more data.
    
    g1 > p1, g2 > p2, p2 > p1
    what to show: g2 > g1 (need more assumption and context to prove it!)
    naive: if p1 is aggregated in the same way as p2 does, we call the resulting model is t1, then maybe we can show g2 > t1, then we need to show t1 > g1, this is because the difference between t1 and g1 is that in t1, p1 is aggregated with more better other clients.
                   
                   
    Another model: probabilistic model:
    with high probability, participating will make you better.
    
    probabilistic result more reasonable.

\end{comment}

The traditional federated learning aims to collaboratively learn a global model that performs well in a universal/global data distribution. However, we argue that distributing every client the exact model is not a good way to incentivize clients. In traditional federated learning, a client who contribute more data can not benefit more than the client who chooses to contribute less data. On the contrary, those clients who contribute less data/model actually benefits more than those who have more contribution. In that sense, we 


Problem Formulation and assumption:
\begin{itemize}
    \item More data, better local model
    \item When a model is aggregated with one more other model, the aggregated model will be better.
    \item when one model is aggregated with a pool of models, if one of the model in the pool is replaced with another better, the aggregation results will be better.
    \item Maybe consider how smooth(weight decay) will affect the performance.
    \item unwillingness to directly share data.
\end{itemize}

\begin{comment}
improvement, if you contribute most, but improvement is the least, you want to quit!

How to make sure you are contribute more, your improvement is also the most, or at least above average?

Compensation? Money? Small hospitals collect money to compensate the big hospitals.

Information asymmetric: if you don't know other's information or maybe only know partial information.

Scenario1:
    A>B>C, participate individually, A's reward seems to be the smallest
Scenario2:
    (B+C)>A, A's reward seems to be the largest.
    how to resolve scenario 2.
    Here, the problem is B is willing to cooperate with C so that even though C will be the one that is benefited most, B could also be benefited from there. In this scenario, A will benefit least even though it has the most data.

Problem:
1. performance improvement ranking hard to be consistent with contribution
2. private cooperation(very natural, maybe don't have to worry too much)
    Counter Argument: maybe only know partial information, 
    1. B does not know how large A's data is
    2. and does not know every other client in the market, maybe even if B merge with C, still does not benefit itself, maybe only boost C. Therefore, C has to 
    3. when B combine with C, C play tricks, only contribute partial data, then after get a model, C fine tune to get a better model.
    
Formalize: if all clients use just traditional federated learning, can cheat. If B and C use federated learning, their incentive can also mismatch. Defeat A's effort is destined to fail!

Law does not allow direct data sharing?


私下采用federated learning会互相欺骗。
私下采用我的mechanism和 总体mechanism没区别？

所有都要归根到utility function, performance is not the only goal!!!

weird to use ranking as a constraint.
cost associated with ranking. higher ranking give higher benefits.


不愿意贡献data原因：1； computation cost low
2. competitiveness increases。不贡献然后再finetune可以让自己利益最大化，比其他人model 都好。

Is there natural consideration to avoid B to join C?

Need to know information of the whole market?

Need to consider fine tuning. 

Everyone's goal: not to maximize performance.

The extreme case we want to avoid: use fake data to steal the global model, then use own data to fine tune.

In the end: benefit depends on 2 things:
1. performance related
2. ranking
(utility should be on that)

Utility function: if only focus on performance, in the traditional federated learning, all the clients will contribute all their data.

Step 1:
We need to design a utility function to incorporate the competitiveness between clients so that they will not always willing to provide all their data in order to maximize their utilities for traditional federated learning, but client will potentially provide more data(maybe all data) given our proposed incentive mechanism.

mechanism involving money is easier than without money.
motivation: 肾脏移植，not permit to involve money.

Solution: U = p + (something depending on partial knowledge of others， alpha * (ranking change))

每个人都不愿意自己的ranking下降。 term：不参加或少参加排名会下降。

(candidate: U = p +() - computation cost) (computation cost is enough to 否定traditiaonl federated learning, 为了省电，moral hazard已经出现， 但是只有computation cost可能解决不了senarior 2)

\begin{equation}
    U_i = performance(d_i, d_{others}) -\beta cost(d'_i) = (d_i + d_others)^\alpha -\beta d'_i
\end{equation}


in utility function, could make P as a lower degree, like square root, make computation cost a nearly linear function, in this case, people are willing to contribute data, but when they contribute a lot, the marginal utility gain is low. Therefore, If we just use traditional federated learning, they are not willing to contribute as much data as possible, because at some point, their marginal cost is larger than the marginal utility(here, we should also model how the federated aggregation affect the utility function, e.g. something like worse than traditional machine learning?)

Another problem here is clients don't know others' data amount, so it's hard to measure their performance in order to calculate the utility value.

However, if we use our own mechanism, clients are willing to contribute more data, since we federated better clients with more other better clients. We should prove it in math formally. We can show that clients marginal utility is almost always larger than the marginal computation cost? Or more likely than before when using just traditional federated learning?

However, we still is likely to have private cooperation issue. However to modify utility function to avoid it?




The problem is if we use 

interesting problem: mechanism design出来以后，如果能prove用了我的mechanism之后，大家ranking不会变，已经足够证明大家都愿意用我的mechanism。
利用无知，每个人都不知道自己是不是最后一个，所以不会造反，而mechiansm依然能保证他参与能获利。
有知：知道mechanism的property（保持ranking）
无知：不知道自己的具体ranking
两者相结合，会incentivize每个人都参与。

Challenge: how to define client's partial knowledge about others?
One Solution: may know a rank(it is easy to know the scale of the hospital, but not the true available total data size).

Step 2:
We need to design a incentive mechanism to make sure that clients are willing to provide their data as much as possible to maximize their new utility function, (considering private cooperation as well)


explore industrial organization.(pricing) cooperate to do R&D. 

Why 2 companies R&D: more than 2 companies, there are others. 
   
Counter Argument, A is also willing to combine with B or C, so in the end, all 3 combine together? So all 3 achieve better rewards(performance improvement) than not joining with others.

In the end, everyone combines together to learn one single shareable model, so there is no federated learning.

We somehow need to provide a term in utility function to force them not to cooperate, (privacy budget), or ranking consistency?

Utility = f(performance improvement, ranking consistency(market standing)) ?

loses competitiveness

how to model selfishness?

\end{comment}
    
\begin{equation}
    U_i = performance(d_i, d_{others}) -\beta cost(d'_i) = (d_i + d_{others})^\alpha -\beta d'_i
\end{equation}
    
\begin{comment}
Improvement. 
Traditional Federated learning, already get the best model.
Utility function: not only client's own performance, but also some fairness.
paradox: only consider own improvement. 
Optimize competitiveness, compared with others.

Common in traditional economy problem (cooperate and compete at the same time).

Either define a utility function: a combination of individual performance improvement and ranking.
    
    

Transparent, could get access to the analysis

Consider every clients tolerance to fairness, if not fairness to some extent, not participate. He can perceive. 

model = f(self data, g(data1), h(data2))

weak monotone, if we have better data, wouldn't be worse.

 the performance of the model is a function of 
 
 every model is a function, monotone function
\end{comment}
 
\begin{comment}
Problem: based on this model assumption, seems that in traditional federated learning, a client could also benefit by contribute more.
\end{comment}



The main idea behind our approach is to distribute models with different quality to the clients based on the the data or model they contribute to participate in the federated learning. Meanwhile, we want to ensure every client is benefited by participating the federated learning, that is, every client is more likely to obtain a better model by participating federate learning than the model after individual training.

\begin{equation}
    ModelPerformance = f(Self Data, g(Data1), h(Data2))
\end{equation}

model performance is a monotone function of data. 
\begin{comment}
But it does not model the case when client merge their data.
\end{comment}

Neighborhood client selection.

We have two requirements, one is the similarity requirement, and the other is fairness requirement.
Clients with better data that results in a better local model should be collaborate together more closely. Moreover, the clients with  better data should collaborate with more clients to improve the model generalization.

To ensure the first requirement. we need to evaluate the "similarity" between different users. We first assume centralized server has access to a universal validation dataset, whose distribution is close to the global data distribution. We then rank each client model on the validation dataset.

If there is no validation dataset, we will measure the distance.

Aggregation method: weighted federated averaging. In the aggregation of each client, the aggregation weight is calculated based on the distance from the other neighborhood client model distance.

Two parameters we would like to address is: weight decay, decay of weight decay. Decay of the aggregation size. The latter two are only for the case validation dataset is available since we can estimate which client has better/model with better quality.

To ensure the fairness requirement, better models need to be aggregated with more other similarly "good" models while worse models should be aggregated with smaller number of worse "bad" models. 

Our assumption: 
1. aggregating with more models is more likely to improve performance

2. aggregating with better models is more likely to benefit than aggregating with worse models.



Therefore, we 

Lemma 1. every participation round improve could improve the model with high probability.

From lemma 1, we can prove that skip rounds cannot cheat. You need to participate as much as possible.

Theorem 1. The better quality your data have, the better your model will be after the federated learning.

Theorem 2. With high probability, the client could obtain a better model than individually training the model.


In our experiment, we use dataset(maybe noisy level, or the level of being backdoor attacked) to measure data quality.
When we use the dataset for data length quality measurement, we need to argue that the many other approaches directly assumes clients honestly report their true datasize, which is not realistic and too ideal. Usually the centralized server is not provided with such information and it has to decide the quality of data through validation test.

\begin{algorithm}
    \caption{Incentive Federated Learning}\label{Alg:Iter}
    \hspace*{\algorithmicindent} \textbf{Input: initial $\theta$, CLIENTUPDATE, SERVERUPDATE} 
\begin{algorithmic}[1]\\

%\Procedure{cyclic training with KNN label correction}{}\\
%\Input{Noisy Training Set $\tilde{S_n}$, $k$, number of epochs \textit{E}}\\
%$\hat{S_n}\leftarrow \tilde{S_n}$\\
\\
\textbf{for} each round t = 1, \textit{M} \textbf{do}\\
\hskip1em Sample a subset $S$ of clients\\
\hskip1em \textbf{for} each client $i \in S$ \textbf{in parallel do}\\
\hskip2em  CLIENTUPDATE()\\
\hskip2em  Client uploads model parameters to the server\\
\hskip1em \textbf{end for} \\
\hskip1em SERVERUPDATE()
\end{algorithmic}
\hspace*{\algorithmicindent} \textbf{Output:} a list of models with different parameters for corresponding clients.
\end{algorithm}

\begin{algorithm}
    \caption{CLIENTUPDATE}\label{Alg:Iter}
    \hspace*{\algorithmicindent} \textbf{Input:} 
\begin{algorithmic}[1]\\
\textbf{for} k=1,...,K \textbf{do}\\
\hskip1em $\theta_{k} \leftarrow OPT(\theta_{k-1},)$
\end{algorithmic}
\hspace*{\algorithmicindent} \textbf{Output:} 
\end{algorithm}

\begin{algorithm}
    \caption{SERVERUPDATE}\label{Alg:Iter}
    \hspace*{\algorithmicindent} \textbf{Input:} 
\begin{algorithmic}[1]\\
$Acc \leftarrow \{\}$\\
\textbf{for} each client $i \in S$ \textbf{in parallel do}
\\
\hskip1em Test model with parameters $\theta_i$ on the validataion dataset, obatain accuracy $Acc_i$ \\
\hskip1em $Acc \leftarrow \{Acc_i\} \bigcup Acc$ \\
\textbf{end for} \\
Sort $Acc$ and rank local client models based on the sorting results.\\
Calculate model weight according to Eq.~\ref{Eq:Aggregate}
\hskip1em 
\end{algorithmic}
\hspace*{\algorithmicindent} \textbf{Output:} 
\end{algorithm}


Our approach works as follows. In each round, all the clients train their own models for multiple epochs. Then clients upload their model parameters to the centralized server. The server samples a certain fraction of clients for aggregation in every round. In our IncentiveFL, the server performs different aggregation weights for different sampled clients based on their individual model performance on a small validation dataset owned by centralized server.

The server will evaluate the performance of the model from each sampled client. Then, all the individual models will be ranked according to their performance on the small validation dataset. Then the higher the client model ranks, the more model parameters will be involved in the weight aggregation so that the aggregated model is supposed to perform better.

The weight will be normally distributed with the centered at clients own position. The weight decays as the other client's rank is further away from the center position among the ranked list. It can be formulated as follows:

The higher data quality the client contributes, the better the local model will perform on the validation dataset, the higher the client will be ranked, the more other models will be aggregated together with the client's model, thus achieving a even better model in general.

\section{Client Model Quality Measurement}

Accuracy, loss, contribution using shapley value. If no valuation dataset is available, we can also use the distance from each model to the global model to rank clients.


\begin{equation}
    w_i =  \sum \alpha * w_j
\end{equation}


\begin{equation}
    l = \min\limits_{\theta} \mathcal{L}(f(\mathbf{x}^t, \theta), y^t)
\end{equation}
Our notion of () is to formalize the the standard intuition that

\begin{equation}\label{Eq:Aggregate}
    \min\limits_{n}
\end{equation}

The key insight is 



Tradeoff between general accuracy and incentives

\subsection{Neighborhood Weighted Aggregation}

\subsubsection{distance metrics}
Distance metrics:

contribution value function.
Possible options:
1. reported data size
2. accuracy measure meant
3. shapley value ~\cite{wang2020principled}

when validation dataset is available, we can do accuracy measurement.

If not, we can collect reported data size from each client.

honest dishonest, report loss, data size, accuracy?

\subsubsection{Weight Parameter}
When valuation dataset is available, we add a weight decay to ensure better client models are aggregated with more other good client models in a smoother way.

\subsection{Performance-Incentive Tradeoff}
Both traditional federated learning and individual learning can be regarded as a special/extreme case of our method. When clients are not collaborating, the fairness is achieved 
We can make a balance between performance and incentive 

==> src/old_algorithm.tex <==
\section{Potential other directions}
\begin{enumerate}
    \item prevent free-ride attack, or how to improve the plain even disguised free-ride attack proposed in the paper. Not simply gaussian noise to the data. Maliciously perturb the model that does not detoriat the model but does not reveal any information.
    \item federated noisy training. Every client has different noisy level. Centralized server determines more reliable agents based on accuracy on a validation dataset.
    \item byzantine, 1/3 is malicious
    \item imcomplete information, does not the the data quality of each client.
\end{enumerate}

\section{Formalized Problem Formulation}

The utility function is composed of privacy and model performance. 

\begin{equation}
    U(p, m) = -p(D_{client}) + m(D_{total})
\end{equation}
$D$ represents the data that clients used to participate the federated learning. Function $p()$ can simply be a linear function, e.g. $p(D) = \gamma|D|$. Function $m$ is definitely much more complicated. But $m()$ generally increases as $|D|$ increases.  It behaves to some extent like a log function. Relation between sample complexity with generalization error: https://arxiv.org/pdf/1712.00409.pdf

\begin{equation}
    \epsilon(|D|) \sim 
    \alpha |D|^{\beta_g}
\end{equation}
with exponent $\beta_g = $ -0.5 or -1. $\epsilon(m)$ is the generalization error.

We assume $p$ and $m$ are linear function of the model performance.
\begin{align*}
    p(D) = \gamma(1-\epsilon(|D|)) \\
    m(D) = \alpha(1-\epsilon(|D|))
\end{align*}


Then we could have a very simply utility function
\begin{equation}
    U_i(p, m) = U_i(D_{total}) =  - \gamma(1-\theta |D_{client_i}|^{\beta_g}) + \alpha(1-\theta |D_{total}|^{\beta_g})
\end{equation}

In the most simple setting, we can assume $\gamma = \alpha$, then we have 
\begin{align}
    U_i(D_{total}) & = - \alpha(1-\theta |D_{client_i}|^{\beta_g}) +\alpha(1-\theta |D_{total}|^{\beta_g})
    \\ & = \theta(|D_{client_i}|^{\beta_g} - |D_{total}|^{\beta_g})
    \\ &  = \theta(|D_{client_i}|^{\beta_g} - \sum_j |D_{client_j}|^{\beta_g})
\end{align}

Take the derivative with respect to $|D_{client_i}|$

\begin{align}
    \frac{\partial U_i}{\partial |D_{client_i}|} & =\theta \beta_g(|D_{client_i}|)^{\beta_g -1} - \theta \beta_g(\sum_j |D_{client_j}|)^{\beta_g -1} \\
    & = \theta \beta_g (|D_{client_i}|^{\beta_g -1} - (\sum_j |D_{client_j}|)^{\beta_g -1}) \\
    & = \theta \beta_g (|D_{client_i}|^{\beta_g -1} - (|D_{client_i}|+\sum_{j\not = i} |D_{client_j}|)^{\beta_g -1})\\
    & < 0 \ \ \ \ since \ \beta_g -1 < 0
\end{align}

Centralized server will set price for the client to buy models. How to set?

Possible directions to explore?
\begin{enumerate}
    \item Can we divide clients into different levels/ranges based on their contribution of data? Each level/range receives a model? If so, can we also involve money. Or maybe, in the extreme case, create different models, set price of each one. The client have the choice to buy specific model based on his interest.
    \item What if clients can leave earlier, can arrival late, can skip iterations. How should the penalty be designed?
    \item It seems in our case, we assume the clients does not know each other's utility, and the centralized server does not know the client's utility function either(maybe they can calculate). Is it something different existing work? Perhaps we are not having a Stackelberg game if centralized server is not a participant, the  information of different clients by-pass the centralized server and is reflected in the utility function of clients. Can we design a game among clients.
    \item How to design better utility function.
    \item what about decentralized setting?
    \item we should consider temporal feature
    \item pretend to participate? solved! solution: add penalty into the price;
    \item model iteration number into the utility.
    \item Clients in our framework are interested in the global model performance.
    \item federated learning to free market learning: don't care server or client. Free market. Client: buy model from market, then train use personalized/local data, then sell them.
    \item if price too high, participants will not participate since they don't have enough data to keep the price low so that they can afford it. So we have to be careful about the price setting.
    \item issue in utility function: they don't now how much data is used by others, so they potentially cannot directly use the size of other's data to approximate the global model performance. They need the centralized server to calculate the performance for them. But for themselves, they don't have a proxy dataset so that they cannot validate their personalized model performance, thus needs to approximate the model performance using the proposed estimation proposed by existing works.
    \item maybe we can first solve the non-iterative case, and then solve the iterative case. In the iterative case, can we assume clients are using the same data in all iterations. If not, we should change the utility function. If centralized server do federated averaging but don't know the data size used for all the clients, it needs to test on proxy dataset to calculate the weight for aggregation.
\end{enumerate}
1. Can we divide clients into different levels/ranges based on their contribution of data? Each level/range receives a model? If so, can we also involve money.
2. What if clients can leave earlier, can arrival late, can skip iterations. How should the penalty be designed?
3. It seems in our case, we assume the clients does not know each other's utility, and the centralized server does not know the client's utility function either(maybe they can calculate). Is it something different existing work?


Price is a function of performance, or something else?


Few assumption in the utility function:
1. size of training data usage and privacy leakage is positively correlated, linearly proportional?

2. model performance is positively correlated with the size of training data usage. maybe lienarly or exponentially proportional?

\subsection{privacy accounting}
Privacy Accounting. In differentially private federated training of DNN models, an important issue arises in accounting for
the multiple iterations of the training algorithm. That is, each participant and therefore each private dataset will be queried during
multiple rounds of training. The composability of differential privacy allows for such iterations to be accounted for by accumulating
the privacy cost at each round of the training as well as the multiple
parameters included in each model update.
To account for the iterative nature of DNN training, the Sequential Composition theorem states that for functions $f_1, . . . , f_n$ where
$f_i$ satisfies $\epsilon$i-DP for each $i \in [1,n]$, the release of the outputs
$f_1(D), . . . , f_n(D)$ satisfies ($\sum^n_{i=1}\epsilon_i$)-DP. The privacy amplification
theorem [4, 14] additionally states that if random samples are selected rather than all available data, then each round satisfying
$\epsilon$-DP incurs only a cost of (q$\epsilon$) against the privacy budget where
q = L/N is the sampling ratio.

Security model. We consider security against honest-but-curious adversaries, i.e., parties following
the protocol but trying to infer as much information as possible about others’ input or function
share.

If not participate in some rounds, there are penalty that adds into the payment they need to make in order to download the global model.


Intuition: without money involved, small data owners and big data owners can never collaborate.

Desired interesting theorem: under this utility assumption, it is impossible to achieve data sharing.

Possible result: if money involved, data sharing becomes possible. Involving money is the only way.

how to get close to the federated learning itself.

write an paper to suggest not only considering engineering/learning, but also considering incentive issue.

cost of Anarchism: traditional problem doesn't consider incentive, the obtained optimal solution is not really optimal. social welfare.
http://www.cs.cornell.edu/~eva/

\section{Problem Formulation}

We are interested in finding a tradeoff between client's model performance and incentive for providing higher quality data.

Assumptions: IID for all clients

Reward determined by performance on aggregated validation dataset.

how can the cheater cheat? 


Things can be done:

Client's side:

1. cheater has no data, reconstruct data, use reconstructed data to train

2. cheater has data, but how to pick T and V. so that uses less T but high score on M


Server's side:
1. implement the baseline ranking mechanism

\section{Main Approach}

Our idea is when performing federated learning, the centralized server personalized the local models, that is, adopting different aggregating strategies for each client so that every client will receive a different model based on the quality of model they sent to the server. 

Assumption1 : the data quantity/quality determines model performance.

Assumption2 : 

Senarios to consider:

1. The client could possibly return the model without any update. If so, what happens to his model in the end

2. If every client do that, what will happen globally in the end.


We draw a comparison between individual learning and federated learning. In individual learning, users can only access their own data so that the individual model performance is determined by the quality of individual dataset. In traditional federated learning, centralized server maintains a global model so that every client can access the global model no matter what quality of data they have. This could be unfair to clients who participates with higher quality data. Those clients who hold little to no data can still obtain a good model from the centralized server. This raises a risk for cheaters/attackers to steal resources without much contribution of good data. Our goal is to make a tradeoff between these two cases so that all the clients will be, to some extent, benefited from participating federated learning while clients who participates with better quality data will obtain more benefit, e.g. get a better model. 

Two extreme cases:

1. individual learning

2. traditional federated learning

Key question: How to make a balance between these two cases?

Can we show that individual client can always benefit from federated learning?


\begin{theorem}
After converged, with high probability, every users can obtain a better model by participating the federated training.
\end{theorem}

\begin{theorem}
After converged, with high probability, if $q_i > q_j$, then $a_i > a_j$
\end{theorem}

where $q_i, q_j$ is the data quality of client i and j. $a_i, a_j$ are accuracy of the model on a global data distribution.

Things to do: mathmatically define $q$, $a$, $dist$

Key problem: how to improve the machanism, use what kind of aggregation approach to adopt.

\begin{lemma}
Weighted aggregation based on distance metrics improves the generalization of the model.
\end{lemma}


In federated learning, the goal is to

\begin{equation}
   C_j = \dfrac{1/dist(W^t_i, W^t_j)}{\sum_{i\not= j}{1/dist(W^t_i, W^t_j)}} 
\end{equation}
where $W^t_i$ represents the model parameter of client $i$ at the $t$th iteration. $C_j$ represents the weight of client $j$'s model during the aggregation to obtain client $i$'s model in next iteration.

Using a distance metric to perform aggregation for each client.

The distance metric can be: model parameter distance, distance between performance among aggregated validation dataset.
Think about: whether with validation dataset is better than without.

Note: Think about how to do the aggregation based on the distance metric. Since it has 0 distance from itself. We cannot simply use inverse of distance to calculated the weight.



\begin{equation}
    W^{t+1}_i = \alpha W^t_i + (1-\alpha)\sum_{i\not = j} C_j W^t_j
\end{equation}

Possible heuristic: do not use all the clients' local models to perform weighted aggregation. could use k-nearest neighbors.

learning rate

auction design mechanism: vickery

https://en.wikipedia.org/wiki/Vickrey%E2%80%93Clarke%E2%80%93Groves_mechanism

Can we involve money/penalty? incentive compatible, accurate.

Training with all data, sell model with price based on client's contribution.

If not involving money, hard to get a tradeoff? Impossible theory?

Data market. many drawbacks. mostly sell raw data. has privacy issue. Now we share model instead of raw data, to some extent, improve privacy.

Narrow down mechanism design space.
Involve money or not?

Havard Eco: https://dash.harvard.edu/bitstream/handle/1/2580565/Roth_kidneyexchange04.pdf?sequenc %3D4


Simple model : DNN perforamcne relation with dataset quality

data solicitation.

If using money to perform iterative federated learning, we should consider the cheater can steal the model from the second last iteration, where the model is close to the final model. Therefore, we need make sure either in each iteration, the model is different for each client based on their data contribution. Or, in each iteration, we should already involve money to make it fair for every client instead of involving money in the very end. 


Money iterative, back and forward all involve money, price determined by performance?

In each iteration, use a proxy dataset to evaluate the performance of the model, then set the price based on the performance. If performance is better, the price is lower. The price is inverse proportional to the performance.

If there is no proxy dataset, we can compute the distance between the averaged model with individual uploaded model. The smaller the distance, the cheaper the price? The distance metric is flexible
Is there any weakness for this mechanism? 
\begin{enumerate}
    \item Too many money transaction, not efficient. 
    \item The attacker can basically skip the early iterations and only participate the very late phase of training so that he doesn't have to pay much to get a good model. Solution: 1. set up the participant pool at the beginning of the training; 2. if someone participate late, need to pay some penalty fee.
    \item Even if every client is required to participate from the very beginning, attacker might still attack? Needs to think
\end{enumerate}

Could we also add the choice such that if the client is willing to pay more, then he can get a better model in each iteration?



Utility involves an additional type of reward: money.
Previous, utility is composed of model performance plus privacy. Now is composed of these two plus money. 

Is it possible to not involve money? why?


incentive compatibility: prove in this mechanism, the best scenario is every client cooperates and contributes as much data as possible.

If the price difference dominates privacy and model performance difference in the utility function, then the best scenario is client contributes as much data as possible.

Nash equilibrium? Definition: a stable state of a system involving the interaction of different participants, in which no participant can gain by a unilateral change of strategy if the strategies of the others remain unchanged.

Can we model more uncertainty? in the assumption, relation between data contribution and model performance?

Next step: move to peer to peer. can involve blockchain.

Different client data distributions: Homo distribution, hetero distribution/each client only hold 1 class of data.



New idea:

gamble, willing to pay how much, center will tell each client how much total bets are against him and how much bets are for them. Based on that, how do they decide the bet they are willing to provide? If their bet depends on the others, what we should do?

Solution: not concurrent bet, assume sequential bet


GAN: How to convert 



Combining federated learning with gamble:

1. utility function is tricky
2. based on existing bets made by earlier participants, the current client will make another bet based on the evaluation of how many total bets are against him and how many bets are with him by providing one data sample to the centralized server along with his own model.


Every time, one client provides one data sample and his own model to the server, server then evaluates how much total earlier bets are against him, how much are for him. Then give him that information, let him decide his own bet. Then how much will he bet?

In the end, the total bets will be distributed to clients that are correct in one sample prediction(maybe make it more to reduce variance).

Possible problems:
1. How to do it iterative?
2. Is this approach robustness, it there any chance someone can cheat in this mechanism?

Who will go first? is it always better to go late?

==> src/old_introduction.tex <==
\section{Introduction}
\iffalse
You Li's thoughts:

Objective:

To enforce that each node cannot change its training set T from the first epoch.

Assumption:

Either with central server, or use P2P communication. In either way, each node will only send out a gradient on the real model for that epoch, plus some results on the auxiliary model. The latter does not affect model accuracy.

Approach:

In each epoch, each party should train the real model and a very small auxiliary model. First, the auxiliary is a "slice" of dimensions of the real model, or it shares some very good property with the real model; so it is verifiable with a particular confidential level, that the gradient trained on the real model can be \textbf{bind} to the gradient or some other computable values on the auxiliary model.

Second, it can be proved using the auxiliary model and the gradient on the auxiliary model, that T is not changed. Potentially here we use ZKP, crypto, or just some empirical results of deep learning.

\fi

A lot of papers approach the incentive problem through reward/money. Our goal is to implicitly incentivize the clients without involving money.

Some interesting findings: The impact of data quality(especially the dataset size) over the client model performance is reflected at the early stage of the training. When the model is already saturated, large dataset size may reversely hurt the model. Therefore, our approach is effective since we look at the individual contribution at the very beginning the training to distribute models for each client. So it's very possible the performance will diverge quickly across clients with various data quality.

Two requirements: 
1. high contributor is more likely to receives high payoff(which, in our framework is get a better model)
2. Clients is more likely to benefit from participating(maybe be not requirement, we can argue this is actually an assumption for clients to participate).
3. The more rounds you participate, the more you improve? lemma: every time you participate, you improve a little bit.

Do we care about the global performance? or personalized performance. If we mainly care about the global performance, maybe we can argue that the performance will also be better when participating federated learning.

Motivation, drawback in traditional federated learning

Potential Problem: don't update but return the trained model? will not improve, if keeping this strategy, client will improve little every time he participates.

What if skip multiple rounds: not problem, your model will be bad.

Give an example of no consideration of incentive when performing federating learning: two player same amount of data, one can cheat, hide his own data, use all fake data. Show that cheater has high benefits,

Traditional federated learning assumes that all the clients are willing to provide their whole dataset but ignores the incentive issue. In reality, it is possible that clients will only provide a small portion from all the data they hold in order to protect their privacy. In principle, the global model will have the best generalization performance if all the client provide all the their data. There is a internal tradeoff between performance and privacy. Some clients could use partial data to participate the federated training. After the joint training finishes, those clients can download the shared global model and finetune on their own whole dataset. In this way, they protect their data privacy while not sacrificing too much performance if most of the other clients are benign. However, if every client does not have the incentive to provide data, the federated training will be no better than individual training since the joint training part become is useless or even harmful while only the local tuning is effective to build useful models. In this sense, if client has little to no incentive to contribute their own data, the federated learning is leaning toward individual learning. 
Our ultimate goal is to build a mechanism that can boost client's incentive to contribute more data when participating federated learning.

Let us consider a simple setting where there are only 2 client2 participating federated learning.
If both clients contribute all data, then the learning exactly like federated learning. If only one of them contributes while the other hides most of data, the one who does not contribute much will get a model with similar performance as the one from the traditional federated learning while the one who actually contributes is benefited no more than individual learning. If none of them is willing to make much contribution, then they become individual learners since the cooperation part does not help.


Utility function: composed of privacy budged/preservation and model performance.


Traditional federated learning without incentive: turns on the best strategy is individual learning. 
Move towards a federated learning goal so that clients are willing to cooperate.

Bonus reward?


\section{Related work}

FAIR RESOURCE ALLOCATION IN FEDERATED
LEARNING, this one talks about fair resource(computation power) while we focus on data fairness.



https://arxiv.org/abs/1905.07479

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8832210&casa_token=o321FElGdv8AAAAA:ebMzAfaZPy47Bz7wsABO47v3Io7dujyGbwmB0z3UipoPw_PneWwx2Cl2jFF0_QGCgo6aDzNsHDw&tag=1

https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9006327

https://arxiv.org/pdf/2002.11711.pdf

https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8875353

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9094030&casa_token=gA_drbatax8AAAAA:6vRuQ0M1vORmwen-xdl3J7mLHhVYFUiaR8d15S0dY6cTfS-lRgyrDKlVSl8naTKQeICjVNgdBU4

https://arxiv.org/pdf/1911.05642v1.pdf

https://pdfs.semanticscholar.org/26a1/8835ac049d65d80fe1e989ae53f3b4760ceb.pdf

https://arxiv.org/pdf/2006.00511.pdf

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9057543&casa_token=n0HcevydWLsAAAAA:qPXgb4WdEMAlhRC4puHdggV35DsJJccWD-FHrG1Kyufax5tEHWwSkEp9IYN0bcFjgvKiQvbt1pA

https://dl.acm.org/doi/pdf/10.1145/3375627.3375840
